MuSR: Testing the Limits of Chain-of-thought with Multistep Soft Reasoning

While large language models (LLMs) equipped with techniques like chain-of-thought prompting have demonstrated impressive capabilities, they still fall short in their ability to reason robustly in complex settings. However, evaluating LLM reasoning is challenging because system capabilities continue to grow while benchmark datasets for tasks like logical deduction have remained static. We introduce MuSR, a dataset for evaluating language models on multistep soft reasoning tasks specified in a natural language narrative. This dataset has two crucial features. First, it is created through a novel neurosymbolic synthetic-to-natural generation algorithm, enabling the construction of complex reasoning instances that challenge GPT-4 (e.g., murder mysteries roughly 1000 words in length) and which can be scaled further as more capable LLMs are released. Second, our dataset instances are free text narratives corresponding to real-world domains of reasoning; this makes it simultaneously much more challenging than other synthetically-crafted benchmarks while remaining realistic and tractable for human annotators to solve with high accuracy. We evaluate a range of LLMs and prompting techniques on this dataset and characterize the gaps that remain for techniques like chain-of-thought to perform robust reasoning.

==> algorithms/_algo_from_contrastive_ex.tex <==
\begin{algorithm}[h!]
\small
\caption{The main search function with a heuristic using the deductive additivity property. Given a set of premises and a goal claim, generate intermediate deductions until the claim is proven true or a termination criterion is met. $E$ is a sentence encoder.}
\begin{algorithmic}
\State {\textbf{Input} A list $X$ of string premises $\mathbf{p}_i$ that will be used to search over to prove a string claim $\mathbf{g}$ }
\State {\textbf{Output} A list of steps taken by the algorithm with their generations}
\State {\textbf{Procedure} $\textsc{Search}(X = \{\mathbf{p}_1,\ \dots\ \mathbf{p}_n\},\ \mathbf{g})$:}
\State $f \gets \{E(\mathbf{p}_i) + E(\mathbf{p}_j)\ |\ \mathbf{p}_i, \mathbf{p}_j\ \in\ X,\ i \neq j \}$
\State $\hat{g} \gets E(\mathbf{g})$
% \State $visited \gets \{\}$
\State $gens \gets \{\}$
\State $maxSteps \in \mathbb{N}$
\State $i \gets 1$
\While{$|f| > 0 \wedge i \leq maxSteps$}

    \State $step \gets \argmax\limits_{x_i \in f} M(x_i, \hat{g})$
    \State $f \gets f\ \setminus\ \{step\}$
    % \State $visited \gets visited\ \bigcup\ \{step\}$
    \State $\text{sample}\ \mathbf{y}_i\ \text{from}\ p_S(\mathbf{y}\ |\ step)$
    \If{$\mathbf{y}_i \notin gens$}
        \State $gens \gets gens\ \bigcup\ \{\mathbf{y}_i\}$
        \State $\textbf{yield}\ (step, \mathbf{y}_i)$
        \If{$\text{entails}(\mathbf{y}_i, \mathbf{g})$}
            \Return
        \EndIf
        \State $\begin{aligned} f \gets f  \cup \{ E(\mathbf{y}_i)\ +\ E(\mathbf{x}_j)\ | \mathbf{x}_j \in X \} \end{aligned} $
        \State $ f \gets f \cup \{ E(\mathbf{y}_i)\ +\ E(\mathbf{y}_j)\ |\ \mathbf{y}_j \in gens, 1 \leq j < i \} $
       
        \State $i \gets i + 1$
    \EndIf
    
    % \State $\begin{aligned}f \gets \{x_i\ |\ x_i\ \in\ f, \argmax\limits_{v_j \in visited} M(x_i, v_j) \leq \alpha \}\end{aligned}$
    
\EndWhile
\end{algorithmic}
\label{alg:ar_search}
\end{algorithm}


==> algorithms/creation_algo.tex <==
% \begin{algorithm}[h!]
% \small
% \caption{Recursive function for creating and validating deductions along a templated tree.}
% \begin{algorithmic}

% \State {\textbf{Input} Templated tree $T$, Generation model $M$, a list of validators $V$, and a prompt template for each deduction $P$ }
% \State {\textbf{Output} A tree filled out with deductions $T'$}
% \State {\textbf{Procedure} $\textsc{CompleteStructure}(T, M, V = \{\mathbf{v}_1,\ \dots\ \mathbf{v}_n\}, P)$:}
% \State $T'.nodes \leftarrow \{RecursivelyDeduce(n_i, M, V, P) | n_i \in T.nodes\}$
% \State $return\ T'$


% \end{algorithmic}
% \end{algorithm}



% \begin{algorithm}[h!]
% \small
% \caption{The function that prompts for a deduction, validates it, then recursively calls itself until all deductions are filled. \zayne{TODO: Validators are not being used currently}}
% \begin{algorithmic}

% \State {\textbf{Input} A node to fill in $n$, A Generation model $M$, a list of validators $V$, and a prompt template $P$ }
% \State {\textbf{Output} A node with its values filled in for the deduction $n_i'$}
% \State {\textbf{Procedure} $\textsc{RecursivelyDeduce}(n_i, M, V = \{\mathbf{v}_1,\ \dots\ \mathbf{v}_n\}, P)$:}
% \State $prompt \leftarrow P(n_i.parent, n_i.children)$
% \State $raw\_deduction \leftarrow M(prompt)$
% \State $n_i' \leftarrow ParseDeduction(n_i, raw\_deduction, M)$
% \If{$n_i' = None$}
% \State $n_i.children \leftarrow \{\}$
% \State $return\ n_i$
% \EndIf
% \While{$|V| > 0$}
% \State $v_i \leftarrow V.pop()$
% \State $valid \leftarrow v_i(n_i')$
% \If{$!valid$}
%     \State $retry\_prompt \leftarrow v_i.prompt\_fn(n_i)$
%     \State $n_i' \leftarrow ParseDeduction(n_i', M(retry\_prompt), M)$
% \EndIf
% \EndWhile

% \State{$complete\_children = \{\}$}
% \While{$|n_i.children| > 0$}
% \State $c^i_j \leftarrow n_i.children.pop()$
% \State $c^{i'}_{j} \leftarrow RecursivelyDeduce(c^{i}_{j}, M, V, P)$
% \State $complete\_children \leftarrow complete\_children \bigcup \{c^{i'}_{j}\}$

% \EndWhile
% \State $ n_i'.children \leftarrow complete\_children$


% \State $return\ n_i'$


% \end{algorithmic}
% \end{algorithm}




% \begin{algorithm}[h!]
% \small
% \caption{Function that will parse the raw string from the language model into the node format or retry if the parse fails. \greg{this one can be compressed or gotten rid of}}
% \begin{algorithmic}

% \State {\textbf{Input} A node to fill in $n_i$, A string output from a language model $s$, A Generation model $M$}
% \State {\textbf{Output} A node with its values filled in for the deduction $n_i'$}
% \State {\textbf{Procedure} $\textsc{ParseDeduction}(n_i, s, M)$:}
% \State $facts \leftarrow \{\}$
% \State $commonsense \leftarrow \{\}$
% \State $retry\_idx \leftarrow 0$
% \While{$retry\_idx < max\_retries$}
% \State $retry\_idx \leftarrow retry\_idx + 1$
% \While{$|s.lines| > 0$}
% \State $l \leftarrow s.lines.pop()$
% \If{$``Fact''\ in\ l\ \vee\ ``Complex''\ in\ l $}
% \State $facts \leftarrow facts \cup \{l.replace(``Fact'', ``'').replace(``Complex'', ``'')\}$
% \EndIf
% \If{$``Commonsense''\ in\ l$}
% \State $commonsense \leftarrow commonsense \cup \{l.replace(``Commonsense'', ``'')$
% \EndIf
% \EndWhile

% \If{$|facts| == |n_i.facts| \wedge |commonsense| == |n_i.facts|$}
% \State $n_i.facts \leftarrow facts$
% \State $n_i.commonsense \leftarrow commonsense$
% \State $return\ n_i$
% \EndIf

% \If{$retry\_idx < max\_retries$}
% \State $prompt \leftarrow P(n_i.parent, n_i.children)$
% \State $s \leftarrow M(prompt)$
% \EndIf

% \EndWhile

% \State $return\ None$

% \end{algorithmic}
% \end{algorithm}



\begin{algorithm}[h!]
\small
\caption{Here we prompt a large language model for a deduction given a node from the reasoning tree.  We validate the deduction is valid and retry up to some limit.  If successful, we update the node with the values from the LLM otherwise we kill the branch by making it a leaf node.}
\begin{algorithmic}

\State {\textbf{Input} An unset deduction node $n_i$, A deduction prompt $p$, a generation model $M$, and a list of validators $V$}
\State {\textbf{Output} A deduction node $n_i$}
\State {\textbf{Procedure} $\textsc{RepromptUntilSuccess}(n_i, p, M, V)$:}

\State $valid \leftarrow False$
\State $retries \leftarrow 3$

\While{$\neg valid \wedge retries > 0$}
\State $retries \leftarrow retries - 1$
\State $output \leftarrow M(p, n_i)$
\State $parsed\_output \leftarrow ParseLines(output)$
\State $valid \leftarrow \forall_{v \in V}\  v(parsed\_output)$
\If{$\neg valid$}
    \State $p \leftarrow RetryPrompt(p, parsed\_output)$
\EndIf

\EndWhile

\If{$\neg valid$}
\State $n_i.children \leftarrow \{\}$
\Else
\State $n_i \leftarrow n_i.update(parsed\_output)$
\EndIf

\State \Return $n_i$


\end{algorithmic}
\label{alg:deduction_creation}
\end{algorithm}


==> algorithms/mm_di_to_et.tex <==
\begin{algorithm}[h!]
\small
\caption{Here we take the facts produced by the Domain Injection stage and use them to create the gold fact set $F$.}
\begin{algorithmic}


\State {\textbf{Input} A dictionary of information on the victim, $v$, A list of dictionaries per suspect for information on each suspect $S$}
\State {\textbf{Output} A collection of facts, $F$, to use in the Entailment Tree construction stage.}
\State {\textbf{Procedure} $\textsc{MurderMysteryCreateFacts}(v, S)$:}

\State $murderer \leftarrow sample(s_i \in S,\ 1)$
\State $F \leftarrow \{\}$
\For{$s_j \in S$}
\If{$s_j = murderer$}
    \State $F \leftarrow F \bigcup \{$``$s_j[``name'']$ has a motive''$,\ $ ``$s_j[``name'']$ has a means''$,\ $``$s_j[``name'']$ has an opportunity''$\}$
\Else
    \State $F \leftarrow F \bigcup sample(\{$``$s_j[``name'']$ has a motive''$,\ $ ``$s_j[``name'']$ has a means''$,\ $``$s_j[``name'']$ has an opportunity''$\},\ 2)$ \Comment{Innocent suspects will be missing either a means, motive, or opportunity.}
    \State $F \leftarrow F \bigcup \{s[``suspicious\_fact'']$\}
\EndIf
\EndFor

\State \Return $F$

\end{algorithmic}
\label{alg:mm_di_to_et}
\end{algorithm}


==> algorithms/ta_di_to_et.tex <==
\begin{algorithm}[h!]
\small
\caption{Here we take the facts produced by the Domain Injection stage and use them to create the gold fact set $F$.}
\begin{algorithmic}

\State {\textbf{Input} A list of three people $P$ and list of skills $S$}
\State {\textbf{Output} A collection of facts, $F$, to use in the Entailment Tree construction stage.}
\State {\textbf{Procedure} $\textsc{TeamAllocationCreateFacts}(P, S)$:}

\State $F \leftarrow \{\}$
\State $M \leftarrow \{\}$

\State $p_i \leftarrow sample(P)$ 
\State $p_j, p_k \leftarrow \{p_l | p_l \in P, p_l \neq p_i\}$

\State $gold\_assignment \leftarrow \{p_i, \{p_j | p_j \in P, p_j \neq p_i \}\}$ \Comment{one person is assigned to the first skill, the remaining two are assigned to the second.}

\State
\State $scores \leftarrow np.ones([3, 5])$ \Comment{Rows represent people, the first two columns are skills and the last three are relationship scores.}
\State $scores[i][0] \leftarrow random.randint(1, 3)$
\State $scores[j][1] \leftarrow random.randint(1, 3)$
\State $scores[k][1] \leftarrow random.randint(1, 3)$
\State $scores[j][k+2] \leftarrow random.randint(1, 3)$
\State $scores[k][j+2] \leftarrow scores[j][k+2]$
\State

\State $scored\_assignments \leftarrow score(P, scores, gold\_assignment)$ \Comment{Returns a sorted list of all assignments, the gold assignment will always be at the top}

\State $gold\_score \leftarrow scored\_assignments[0]$
\State $second\_best\_score \leftarrow scored\_assignments[1]$
\State $delta \leftarrow gold\_score - second\_best\_score$

\While {$delta > 2$}

\If{$random() > 0.5$}

\If{$random() > 0.5$}
    \State $scores[i][1] = min(3, scores[i][1]+1)$
\Else
    \State $l \leftarrow random.pick(j, k)$
    \State $scores[i][l+2] = min(3, scores[i][l+2]+1)$
\EndIf
    
\Else

\State $l \leftarrow random.pick(j, k)$

\If{$random() > 0.5$}
    \State $scores[l][0] = min(3, scores[l][0]+1)$
\Else
    \State $l \leftarrow random.pick(j, k)$
    \State $scores[l][i+2] = min(3, scores[l][i+2]+1)$
\EndIf

\EndIf

\State $scored\_assignments \leftarrow score(P, scores, gold\_assignment)$ 
\State $gold\_score \leftarrow scored\_assignments[0]$
\State $second\_best\_score \leftarrow scored\_assignments[1]$
\State $delta \leftarrow gold\_score - second\_best\_score$

\EndWhile

\State


\State $skill\_strings \leftarrow [$``bad'', ``okay'', ``good''$]$
\State $relationship\_strings \leftarrow [$``badly'', ``okay'', ``well''$]$

\For{$p_l \in P$}

\State $F \leftarrow F \bigcup \{$``$p_l$ is $skill\_strings[scores[l][0]]$ at $S[0]$.''$\}$
\State $F \leftarrow F \bigcup \{$``$p_l$ is $skill\_strings[scores[l][1]]$ at $S[1]$.''$\}$

\For {$p_m \in P[l+1:]$}
\State $F \leftarrow F \bigcup \{$``$p_l$ works $relationship\_strings[scores[l][m+2]]$ with $p_m$.''$\}$
\EndFor

\EndFor

\State \Return $F$


\end{algorithmic}
\label{alg:mm_di_to_et}
\end{algorithm}


==> algorithms/tom_di_to_et.tex <==
\begin{algorithm}[h!]
\small
\caption{Here we take the facts produced by the Domain Injection stage and use them to create the gold fact set $F$.}
\begin{algorithmic}


\State {\textbf{Input} A list of items $I$, a list of locations $L$, starting locations for each item $S$, a list of people $P$, floating point representing the chance of seeing a move $o$, and the number of moves $m$.}
\State {\textbf{Output} A collection of facts, $F$, to use in the Entailment Tree construction stage.}
\State {\textbf{Procedure} $\textsc{ObjectPlacementsCreateFacts}(I, L, S, P, o, m)$:}

\State $F \leftarrow \{\}$
\State $move\_idx \leftarrow 0$
\State $curr\_locations \leftarrow S$
\State $beliefs\_locations \leftarrow \{p_i: S | p_i \in P\}$
\While{$move\_idx < m$}
\State $move\_idx++$
\State $moved\_item \leftarrow AssignItem(I)$ \Comment{We randomly pick an item that has been moved less than 2 times.}
\State $moved\_location \leftarrow AssignLocation(L, moved\_item)$ \Comment{Random location that is currently not where the $moved\_item$ is.}
\State $mover \leftarrow AssignMover(P, moved\_item)$ \Comment{We randomly pick a person that has not moved twice and that knows the location of $moved\_item$.}

\State{$F \leftarrow F \bigcup \{$``$mover$ moves the $moved\_item$ to the $moved\_location$''$\}$}
\State $beliefs\_locations[mover][moved\_item] \leftarrow moved\_location$
\State $curr\_locations[moved\_item] \leftarrow moved\_location$

\For{$i_j \in \{i_j | i_j \in I, i_j \neq moved\_item$}

\If{$curr\_locations[i_j] = moved\_location$}

\State{$F \leftarrow F \bigcup \{$``$mover$ sees the $i_j$ at the $moved\_location$''$\}$}
\State $beliefs\_locations[mover][i_j] \leftarrow moved\_location$

\EndIf

\EndFor

\For{$p_i \in \{p_i | p_i \in P, p_i \neq mover \}$}
\State $seen \leftarrow random() > o$
\If{$seen$}
\State{$F \leftarrow F \bigcup \{$``$p_i$ saw the $moved\_item$ move to the $moved\_location$''$\}$}
\State $beliefs\_locations[p_i][moved\_item] \leftarrow moved\_location$
\Else
\State{$F \leftarrow F \bigcup \{$``$p_i$ did not see the $moved\_item$ move to the $moved\_location$''$\}$}
\EndIf
\EndFor
\EndWhile

\State \Return $F$

\end{algorithmic}
\label{alg:tom_di_to_et}
\end{algorithm}


==> prompts/tom/rewrite.tex <==
\begin{longprompt}[caption={ToM prompt for rewriting the story into a coherent narrative.},label={lst:tom_story_rewrite_sg}]
Mason, the magician, along with Adam, an intrigued audience member, and Patricia, his assistant, all knew a spectacular performance awaited. All eyes were drawn to the top hat resting peacefully on the props table ready for the magic show. Yet, their hearts were itching for the magic deck of cards, tucked away safe in the backstage room, the true star of this magic performance.
Everyone knew that the top hat was at the props table and that the magic deck of cards was at the backstage room.

Being quite organized, Mason decided to relocate the top hat to the stage.
	Meanwhile, While Mason was dazzling and perplexing the crowd with his mesmerizing disappearing trick, Adam was watching carefully, trying to decipher how the tricks were executed. One trick in particular caught his eye: Mason's vanishing card trick. His sleight of hand during his series of card shuffling tricks seemed almost magical, and Adam was determined to find that hidden card.

As Mason's illusions kept the audience enthralled, Patricia was diligently ensuring his magic costume was properly arranged for his climactic final act. Patricia, through precise hands and sharp eyes, was meticulously adjusting the placement of the sequins on the costume while packing it away into the suitcase. Mason continued to mesmerize the audience with his performance, moving around whilst Patricia paced and packed, her concentred gaze never leaving the suitcase.

Patricia, with a sense of organization, moved the magic deck of cards to the props table.
	Meanwhile, Adam, who had been standing idly by, looked in Patricia's direction just as she fleetingly flicked her wrist. Following this brief exchange, Patricia opted to move elsewhere. Prior to her departure, Mason had indicated to Patricia that a particular card was required. Showcasing his intense focus, all of Mason's attention was directed towards the deck of cards. As Patricia smoothly picked up the deck, Adam's gaze momentarily connected with hers. After all, she was standing right beside Mason when she made her move. Interestingly, the card Mason had mentioned was cunningly hidden at the bottom of the deck.

Mason, preparing for his performance, moved the magic deck of cards to the stage.
	Meanwhile, Adam found himself completely enraptured by the elderly lady's intriguing tales. His deep interest was stoked by her personal accounts of interacting with magic in her past years. The intricacy of the details, particularly those concerning Mason's incredible conjuring tricks, held his undivided attention. Patricia observed the movement of the magic deck of cards onto the stage.
---
The above story was created by generating each paragraph separately.  This was to ensure that no facts were missed when creating the story and to separate key information.  Can you rewrite the above story to have the EXACT information in the EXACT same way; however, make it flow like a narrative.  Fix any continuity errors as well with MINIMAL change to the underlying facts. Each beginning sentence, describing someone moving something, MUST remain in the story.  We will ask readers about where things are placed after they read it, this must be clear.

The story is told sequentially.  Each paragraph should be thought of as restarting the story. What the characters were doing while something was moved previously, is not what they are doing for the current move.  Because of this, every time something is moved, you should explicitly and in detail explain what each person is doing.

Never add additional input to the characters, what they see, or what they know. Ever.

Ensure that all characters know the starting locations of all objects in the first paragraph.  This should already be stated, but if it is not explicit that everyone in the story knows the locations, make it so.

\end{longprompt} 

==> tables/eval_entailment_tree_validity.tex <==
\begin{table}
\small
\caption{Quality metrics for the reasoning questions generated by our algorithm in CMCR.  We find that the deductions are valid N\% of the time and that the majority of facts are entailed by the story they are used to generate.  This ensures the quality and solvability of the problems we generated for CMCR. \zayne{We could break this into two tables, or two graphs.  We could show validity of deductions as we increase the depth of the tree, but we rarely go past d=3; however, it would show that the entailment method scales.  Not a necessary point for this though.}}
%\renewcommand{\tabcolsep}{0.9mm}
\begin{tabular}{c|cc}
\toprule
& \multicolumn{2}{c}{Validity} \\\midrule
Domain & Valid Deductions & Entailed Facts \\\midrule
Murder Mysteries & \\
Object Placements & \\
Movie Recommendations & \\

\bottomrule
\end{tabular}
\label{tab:eval_dataset_quality}
\end{table}


==> tables/eval_facts_only.tex <==
\begin{table}
\small
%\renewcommand{\tabcolsep}{0.9mm}
\begin{tabular}{c|ccccccccc}
\toprule
& \multicolumn{3}{c}{Murder Mysteries} & \multicolumn{3}{c}{Object Placements} & \multicolumn{3}{c}{Team Allocation} \\\midrule
 & Simple & D1 & D1 w/ CS & D2 & D2 w/ CS & D3 & D3 w/ CS \\\midrule
GPT3.5 & \\
GPT-4 & \\
Vicuna/Llama something & \\
\bottomrule
\end{tabular}
\caption{
\zayne{TODO: wrong format / probably a line chart or a line chart with bar chart for cs no/cs. etc.}
Results of the smaller Language Models given facts at various depths of the entailment tree.  The facts are given in a list rather than a natural narrative.  \zayne{This would be cool with any of the models, and it'd be cool to put this in a line graph of some sort.  With tons of models going across.  I don't think we need human eval for this right? If we show the results from the first experiments ``data quality'' they should follow.}  \greg{Possibly comment on the very simple ``Fact 827'' results here, either in the text or explicitly in the table}
}
\label{tab:facts_only}
\end{table}


==> tables/eval_soft_context.tex <==
\begin{table}
\small
%\renewcommand{\tabcolsep}{0.9mm}
\begin{tabular}{c|ccccccccc}
\toprule
& \multicolumn{3}{c}{Murder Mysteries} & \multicolumn{3}{c}{Object Placements} & \multicolumn{3}{c}{Movie Recs} \\\midrule
Domain & D1 & D2 & Full w/ CS  & D1 & D2 & Full w/ CS & D1 & D2 & Full w/ CS   \\\midrule
GPT3.5 & \\
Llama 2 7B & \\
Vicuna 7B & \\
\bottomrule
\end{tabular}
\caption{Results on easier contexts where we generate a story at varying levels of depths in the entailment tree.  We also test the performance of natural contexts when commonsense facts are explicitly stated. \zayne{more about results etc.}\zayne{DROP THIS}}
\label{tab:soft_reasoning}
\end{table}

